CIBER 4th flight fluctuation analysis: Pseudo-power spectrum formalism, improved source masking and validation on mocks

Precise, unbiased measurements of extragalactic background anisotropies require careful treatment of systematic effects in fluctuation-based, broad-band intensity mapping measurements. In this paper we detail improvements in methodology for the Cosmic Infrared Background ExpeRiment (CIBER), concentrating on flat field errors and source masking errors. In order to bypass the use of field differences, which mitigate flat field errors but reduce sensitivity, we characterize and correct for the flat field on pseudo-power spectra, which includes both additive and multiplicative biases. To more effectively mask point sources at 1.1 $\mu$m and 1.8 $\mu$m, we develop a technique for predicting masking catalogs that utilizes optical and NIR photometry through random forest regression. This allows us to mask over two Vega magnitudes deeper than the completeness limits of 2MASS alone, with errors in the shot noise power remaining below $<10\%$ at all masking depths considered. Through detailed simulations of CIBER observations, we validate our formalism and demonstrate unbiased recovery of the sky fluctuations on realistic mocks. We demonstrate that residual flat field errors comprise $<20\%$ of the final CIBER power spectrum uncertainty with this methodology.

==> sections/data_preprocess.tex <==
\section{Data Pre-processing}
\label{S:data_preprocess}

\subsection{Flat field correction and gradient subtraction}
\label{sec:ffgrad}

\richard{Estimate and correct for the flat field responsivity and large-scale gradients. In practice the two are estimated together using the iterative procedure described in \S \ref{sec:ffgrad}. This is done for each detector quadrant separately. }

The second is correction for relative gain variations across each imager, otherwise known as the flat field responsivity. While laboratory measurements utilizing an integrating sphere for uniform illumination with a solar-type spectrum were initially used to estimate the flat field, these measurements were found to be inconsistent with the flat field estimates derived from flight exposures \richard{reference?}. Such differences may be due to the optical configuration of the experiment between lab measurements and flight, differences in the electrical environments (flight data are taken on internal battery power while lab measurements use an external power source). In the absence of a well-determined flat field, \zem\ used field differences to mitigate flat field errors at leading order, as the flat field error primarily couples with the mean normalization of the maps. This error cancellation is spoiled by unequal mean levels between pair-differenced fields. Field differences also make power spectrum de-convolution more difficult due to higher masking fractions (the effective mask is the union of individual field masks), degrading statistical sensitivity and limiting the achievable masking depth for point sources. 

An alternative approach which we pursue in this work is to estimate the flat field from exposures taken during flight. This can be done by stacking the flat field estimates derived from each field that use the mean background, dominated by Zodiacal light, as an approximate uniform illuminator. 


The relative gain estimate for each field comes from stacking the four other science fields (``off-fields") in a round-robin approach.  

\subsubsection{Iterative FF+gradient removal}
The flat field estimator using \emph{CIBER} science fields involves masking out bright sources within each field and then stacking combinations of exposures normalized by their means. While the astrophysical signals will vary across images, the flat field responsivity will not, and so in the limit of many independent exposures this estimator should converge to the true flat field. However the presence of gradients in the stacked fields will bias the flat field responsivity on large scales -- by the same token there is some degeneracy between large scale responsivity variations and sky gradients. We implement an iterative procedure to compute the gradients and flat fields: 

\begin{enumerate}
    % \item Initialize $i=0$
    \item Calculate the stacked flat field estimates for each field $j$:
    \begin{align}
    \hat{FF}^i_{j} = \sum_{j^{\prime} \neq j}\frac{w_{j^{\prime}} I^i_{j^{\prime}}}{\overline I^i_{j^{\prime}}} / \sum_{j^{\prime} \neq j} w_{j^{\prime}}
    \end{align}
    \item Estimate gradients of corrected fields
    \begin{equation}
    G^{i}_j = \mathcal{G}\left[I^i_{j}/FF^i_j\right] \quad \text{for }j=0\text{ to }N_f-1
    \end{equation}
    where $\mathcal{G}$ is the gradient computed with masked flight images.
    \item Subtract the gradient from the FF-corrected image. and Multiply the subtracted image by $FF_j^i$, i.e.,
    \begin{equation} I^{i+1}_j = FF^i_j\left[\frac{I^i_j}{FF^i_j} - G_j^{i}\right]. \end{equation}
    \item Go back to (1) and repeat.

\end{enumerate}
At each iteration the impact of large scale gradients on flat field estimates is reduced. Convergence is achieved after a few ($\lesssim$5) iterations as evaluated by the best-fit gradient parameters. The final gradient subtracted by the end of several iterations is typically within 10\% of the single pass estimate, while the flat field differs by less than one per cent. Given the mean normalization of the maps relative to the instrument+photon noise, the per pixel RMS for each of the two imagers is $\sim 10\%$ for each stacked flat field estimates, though because of the round robin approach the flat field for each science field has slightly different noise properties. 

There are quadrant-specific electrical effects which source anisotropic power on large scales. As such, the gradient subtraction at each iteration is performed on separate quadrants of the imager (see \S \ref{sec:filterchoice}). This results in a more aggressive transfer function on the largest scales, however at \emph{CIBER} sensitivity the loss of astrophysical information is relatively minimal. 
